Differentially Private Algorithms for Empirical Machine Learning

An important use of private data is to build machine learning classifiers. While there is a burgeoning literature on differentially private classification algorithms, we find that they are not practical in real applications due to two reasons. First, existing differentially private classifiers provide poor accuracy on real world datasets. Second, there is no known differentially private algorithm for empirically evaluating the private classifier on a private test dataset. In this paper, we develop differentially private algorithms that mirror real world empirical machine learning workflows. We consider the private classifier training algorithm as a blackbox. We present private algorithms for selecting features that are input to the classifier. Though adding a preprocessing step takes away some of the privacy budget from the actual classification process (thus potentially making it noisier and less accurate), we show that our novel preprocessing techniques significantly increase classifier accuracy on three real-world datasets. We also present the first private algorithms for empirically constructing receiver operating characteristic (ROC) curves on a private test set.

==> ROCproof.tex <==
\section{Proof of Theorem 5}
\begin{proof}
All the $TPRs$ and the $FRPs$ can be written as
\begin{eqnarray}
\nonumber
TPR(\theta_{i}) = \frac{TP(\theta_{i})}{TP(\theta_{n})} \\
\nonumber
FPR(\theta_{i}) = \frac{FP(\theta_{i})}{FP(\theta_{n})}
\end{eqnarray}

$TP(\theta_{i}),FP(\theta_{i})$ can be computed by answering all one-sided range queries on the $s_{i}$ sequence we have defined in the previous section.

In our algorithm, we use Privelet method to perturb the $s_{i}$, and the sensitivity for each one-sided range query is $log(n)$. Therefore, given fixed $\epsilon$ and $\delta$, the error between noisy $\tilde{TPR(\theta_{i})}$ and real $TPR(\theta_{i})$ or will be bounded by
\begin{eqnarray}
\nonumber
\lefteqn{|\tilde{TPR(\theta_{i})} - TPR(\theta_{i}) |} \\
\nonumber
&& \leq max \{\frac{TP(\theta_{i}) + Lap(\frac{log(n)}{\epsilon},\delta)}{|P| -Lap(\frac{log(n)}{\epsilon},\delta)} - \frac{TP(\theta_{i})}{|P|}, \\
\nonumber
&& \frac{TP(\theta_{i})}{|P|} - \frac{TP(\theta_{i}) - Lap(\frac{log(n)}{\epsilon},\delta)}{|P| + Lap(\frac{log(n)}{\epsilon},\delta)} \}
\end{eqnarray}

Also, since $TP(\theta_{i}) \leq |P|$, we can get the following inequations
\begin{eqnarray}
\nonumber
\frac{TP(\theta_{i}) + Lap(\frac{log(n)}{\epsilon},\delta)}{|P| -Lap(\frac{log(n)}{\epsilon},\delta)} \leq \frac{TP(\theta_{i}) + 2*Lap(\frac{log(n)}{\epsilon},\delta)}{|P|} \\
\nonumber
\frac{TP(\theta_{i}) - Lap(\frac{log(n)}{\epsilon},\delta)}{|P| + Lap(\frac{log(n)}{\epsilon},\delta)}  \ge \frac{TP(\theta_{i}) - 2*Lap(\frac{log(n)}{\epsilon},\delta)}{|P|} 
\end{eqnarray}

Thus, we can bound the $\tilde{TPR(\theta_{i})}$ by
\begin{eqnarray}
\nonumber
|\tilde{TPR(\theta_{i})} - TPR(\theta_{i}) | \leq \frac{2*Lap(\frac{log(n)}{\epsilon},\delta)}{|P|} = X
\end{eqnarray}

Similarly, we can bound the noisy $\tilde{FPR(\theta_{i})}$ by
\begin{eqnarray}
\nonumber
|\tilde{FPR(\theta_{i})} - FPR(\theta_{i}) | \leq \frac{2*Lap(\frac{log(n)}{\epsilon},\delta)}{|N|} = Y
\end{eqnarray}


Based on the X-axis ($FPRs$), the area of the ROC curve can be computed like
\begin{eqnarray}
\nonumber
A = \sum_{i=1}^{n} (FPR(\theta_{i}) - FPR(\theta_{i-1})) \frac{TPR(\theta_{i}) + TPR(\theta_{i-1})}{2} + bias
\end{eqnarray}

We define some new notations at thresholds $\theta_{i}$,$i = 1,\dots,n-1$
\begin{eqnarray}
\nonumber
\underline{TPR(\theta_{i})}= max(0, TPR(\theta_{i}) - X) \\
\nonumber
\underline{FPR(\theta_{i})} = max(0, FPR(\theta_{i}) - Y) \\
\nonumber
\overline{TPR(\theta_{i})} = min(1, TPR(\theta_{i}) + X) \\
\nonumber
\overline{FPR(\theta_{i})} = min(1, FPR(\theta_{i}) + Y)
\end{eqnarray}

Also we define
\begin{eqnarray}
\nonumber
\underline{TPR(\theta_{0})} = \overline{TPR(\theta_{0})} = TPR(\theta_{0}) = 0 \\
\nonumber
\underline{TPR(\theta_{n})} = \overline{TPR(\theta_{n})} = TPR(\theta_{n}) = 1
\end{eqnarray}

Based on these notations, we can draw the upper bound of the ROC curve by using points ($\underline{FPR}(\theta_{i})$, $\overline{TPR}(\theta_{i})$) and draw the lower bound of the ROC curve based on points ($\overline{FPR}(\theta_{i})$, $\underline{TPR}(\theta_{i})$) at all thresholds. Then, we can bound the area of the lower bound $LA$ and the area of the upper bound $UA$ as
\begin{eqnarray}
\nonumber
LA \ge \sum_{i=1}^{n} (\overline{FPR}(\theta_{i}) - \overline{FPR}(\theta_{i-1})) \frac{\underline{TPR}(\theta_{i}) + \underline{TPR}(\theta_{i-1})}{2} \\
\nonumber
UA \leq \sum_{i=1}^{n} (\underline{FPR}(\theta_{i}) - \underline{FPR}(\theta_{i-1})) \frac{\overline{TPR}(\theta_{i}) + \overline{TPR}(\theta_{i-1})}{2}
\end{eqnarray}

If each $X$ or $Y$ is out of the range (0,1), we only consider the situation that $X$ or $Y$ is above 1 since once $X$ or $Y$ is below 0, it means we add bigger noise than the situation when $X$ or $Y$ is above 1. Thus, the lower bound and the upper bound under situation of ''below 0'' should be even worse than under the situation of ''above 1''. If the $X$ is above 1, $\underline{TPR} = 0$ and $\overline{TPR} = 1$ at all thresholds. If the $Y$ is above 1, $\underline{FPR} = 0$ and $\overline{TRP} = 1$ at all thresholds. (1) is proved.

If both $X$ and $Y$ is within the range (0,1), we first divide all thresholds into two parts
\begin{eqnarray}
\nonumber
P_{1} &=& \{i \mid FPR(\theta_{i}) < Y, i = 0,\dots, N\} \\
\nonumber
P_{2} &=& \{0,\dots,N\} - P_{1}
\end{eqnarray}
$\underline{FPR(\theta_{i})} = 0$ for all $i \in P_{1}$. 

Then, we can compute the error of the area between $UA$ and $A$ as
\begin{eqnarray}
\nonumber
\lefteqn{|UA - A|} \\
\nonumber
&&\leq \sum_{i \in P_{1}}^{} \{(\underline{FPR}(\theta_{i}) - \underline{FPR}(\theta_{i-1})) \frac{\overline{TPR}(\theta_{i}) + \overline{TPR}(\theta_{i-1})}{2}\\
\nonumber
&&- (FPR(\theta_{i}) - FPR(\theta_{i-1})) \frac{TPR(\theta_{i}) + TPR(\theta_{i-1})}{2}\} \\
\nonumber
&&+ \sum_{i \in P_{2}}^{} \{(\underline{FPR}(\theta_{i}) - \underline{FPR}(\theta_{i-1})) \frac{\overline{TPR}(\theta_{i}) + \overline{TPR}(\theta_{i-1})}{2} \\
\nonumber
&&- (FPR(\theta_{i}) - FPR(\theta_{i-1})) \frac{TPR(\theta_{i}) + TPR(\theta_{i-1})}{2} \} + bias\\
\nonumber
&&\leq \sum_{i \in P_{2}}^{} \{(\underline{FPR}(\theta_{i}) - \underline{FPR}(\theta_{i-1})) \frac{\overline{TPR}(\theta_{i}) + \overline{TPR}(\theta_{i-1})}{2} \\
\nonumber
&&- (FPR(\theta_{i}) - FPR(\theta_{i-1})) \frac{TPR(\theta_{i}) + TPR(\theta_{i-1})}{2} \} + bias
\end{eqnarray}  

The following equations are satisfied
\begin{eqnarray}
\nonumber
\lefteqn{FPR(\theta_{i}) - FPR(\theta_{i-1}) = \underline{FPR(\theta_{i})} - \underline{FPR(\theta_{i-1})} }\\ 
\nonumber
&& i \in P_{2} - \{n\}\\
\nonumber
\lefteqn{(\underline{FPR(\theta_{n})} - \underline{FPR(\theta_{n-1})} ) - (FPR(\theta_{n}) - FPR(\theta_{n-1}))} \\
\nonumber
&&= (1 - \underline{FPR(\theta_{n-1})}) - (1 - FPR(\theta_{n-1})) = Y
\end{eqnarray}

Therefore, we can further bound the error as
\begin{eqnarray}
\nonumber
\lefteqn{|UA - A|} \\
\nonumber
&&\leq \sum_{i \in P_{2} - \{n\}}^{} \{(\underline{FPR}(\theta_{i}) - \underline{FPR}(\theta_{i-1}))\\
\nonumber
&&- (FPR(\theta_{i}) - FPR(\theta_{i-1})) \} *X\\
\nonumber
&&+ Y*\frac{TPR(\theta_{n}) + TPR(\theta_{n-1})}{2} + bias\\
\nonumber
&&\leq X*(1-Y) + Y = X + Y - X*Y + bias
\end{eqnarray}

If the computation is based on Y-axis ($TPRs$), we can get the similar result as 
\begin{eqnarray}
\nonumber
|UA - A| \leq Y*(1-X) + X = X + Y - X*Y + bias
\end{eqnarray}
Thus, we prove that 
\begin{eqnarray}
\nonumber
|UA - A| \leq X + Y - X*Y + bias
\end{eqnarray}
Similarly, we can prove
\begin{eqnarray}
\nonumber
|A - LA| \leq X + Y - X*Y + bias
\end{eqnarray}
(2) is proved and the proof for thereom 5 is done
\end{proof}


==> linearization.tex <==
\section{Linearization of IG}\label{sec:linearization}
\todo{linearization proof goes here...}
\begin{definition}[Maximum Joint Distribution]
Given a pair of binary random variables $X, Y$, the maximum joint distribution $Pr*[X, Y]$
\end{definition}
